Composing Text and Image for Image Retrieval - An Empirical Odyssey

In this paper, we study the task of image retrieval, where the input query is specified in the form of an image plus some text that describes desired modifications to the input image. For example, we may present an image of the Eiffel tower, and ask the system to find images which are visually similar but are modified in small ways, such as being taken at nighttime instead of during the day. To tackle this task, we learn a similarity metric between a target image and a source image plus source text, an embedding and composing function such that target image feature is close to the source image plus text composition feature. We propose a new way to combine image and text using such function that is designed for the retrieval task. We show this outperforms existing approaches on 3 different datasets, namely Fashion-200k, MIT-States and a new synthetic dataset we create based on CLEVR. We also show that our approach can be used to classify input queries, in addition to image retrieval.

==> sections/backup/intro-old.tex <==
\section{Introduction}


Recent deep learning models have achieved a remarkable performance in recognizing a variety of objects, animals, scenes,~\textit{etc}. It still remains challenging to recognize complex concepts.
To advance the capability of semantic understanding and reasoning, an emerging research area called compositional learning~\cite{misra2017red} has been gaining some momentum. The core of compositional learning is that a complex concept can be developed by combing multiple simple concepts or attributes~\cite{misra2017red}. The idea is reminiscent of earlier work on visual attribute~\cite{farhadi2009describing,sadeghi2011recognition} and recent studies focus on composting two learned classifiers into a new classifier~\cite{misra2017red,nagarajan2018attributes,kato2018compositional}, \eg composing ``pink'' and ``elephant'' classifiers to recognize ``pink elephant''.

%Introduce the new problem. Why it is important
A natural composition often occurs between texts and images. Consider the example in Fig.~\ref{fig:task}, given a query image and a text description, our goal is to retrieve the relevant image that is visually similar to the query image except for the modification specified in the text. This represents a typical scenario in session search, in which after users find an image, they can use it as a reference or a context, express its modifications in text, and retrieve more relevant images. Language offers a flexible vehicle to express ``difference'' to the image, and hence offering a more expressive paradigm for image retrieval than  traditional image-to-image search~\cite{wang2014learning} or zero-shot learning~\cite{lampert2009learning}. \cs{Maybe find another example than image search? Not sure if it is okay for pub-approval.}



\begin{figure}[t]
\begin{center}
% \includegraphics[width=0.99\linewidth]{res/intro.png}
%\includegraphics[width=0.85\linewidth]{res/intro2.png}
%\includegraphics[width=0.99\linewidth]{res/intro4.png}
\includegraphics[width=0.99\linewidth]{res/fig1.pdf}
\end{center}
\caption{Compositional learning for classification (Top) and for retrieval (Bottom). In retrieval, we only have a single instance of the query image and the composition is between the image and the text.}
   %\caption{Example of how image text composition query can be more expressive for retrieval.}
\label{fig:task}
\end{figure}

% New problem and relation to existing work
To the best of our knowledge, such cross-modal composition has not yet been explored in the context of compositional learning. Our problem is nevertheless related to the following areas. The first is Visual Question Answering (VQA)~\cite{vqa}, in which language and image are integrated for answer inference. A disparity to our work is that the text in VQA is used as a clue to find answer in the image as opposed to as modifications to be made to the query image. Another closely related topic is attribute-based product search~\cite{liu2016deepfashion}, where users can change the attribute of an image to find more relevant products. As we will see, the problem differs from ours in that our text modification is more complicated than a single attribute. In addition, product search seldom shows its effectiveness beyond image retrieval. In comparison, we focus on learning compositional visual-text embedding and demonstrate the state-of-the-art results on the both retrieval and classification task.

% Our approaches and how we address the challenges
In this paper, we introduce a framework to tackle compositional learning for image retrieval. We conduct extensive experiments investigating the behavior of existing composition mechanism in our setting. Numerous empirical observations lead us to propose a novel~\emph{MOdification via REsidual Link (MOREL)} module to learn the visual-text compositional feature, in which the text feature is learned to modify the image feature via a residual link controlled by a learnable gate. It leverages a ResNet architecture ~\cite{he2016identity} to inject feature modification (described by the text) to the reference image feature, and learns to balance between preserving the image feature and applying modification. After getting the modified image feature, we can leverage the standard image-to-image retrieval. MOREL can be integrated in different types of layers in a Convolution Neural Network (CNN). While being used in a convolution or a fully-connected layer, it is able to perform spatial-aware modifications where depending on the query, the modification can be carried out in either a region or the entire image.

% Key results
We empirically validate our method on three benchmarks: Fashion200K~\cite{han2017automatic}, MIT-States~\cite{StatesAndTransformations} as well as a new dataset called CSS. We create CSS from CLEVR~\cite{johnson2017clevr} and make it easy to diagnose under different settings and easy to visualize the learned compositional feature.
Experimental results show that our method performs favorably against existing methods. Though our focus is image retrieval, our method turns out working reasonably well on compositional learning for classification, and achieves the state-of-the-art result on the unseen combination recognition task on MIT-States. The qualitative studies on the new dataset of CSS verify that the reconstructed images by our method are more sensible to humans suggesting the modification is semantically meaningful. Ablation studies are included ...


%The technical novelty of this paper includes
%the solutions in system design and the insight on a
%number of empirical studies on


%\lu{chanhge the contribution to reflect: how we adapt image retrieval pipeline to the new/more expressive query, + investigate a couple of composition mechanisms, + additionally our proposed composition architecture MOREL}
To summarize, our contribution is threefold: 
\begin{itemize}
\item We study the cross-modal compositional learning for image retrieval, establishing a new benchmark and insightful empirical studies using existing composition mechanisms.
\item We propose a novel, simple, yet effective composition mechanism named MOdification via REsidual Link (\fancyname).
\item Extensive experiments verify our method performs favorably against strong baselines, achieving the best published results on two public benchmarks Fashion200K and MIT-States. Ablation studies are presented to verify the contribution of the proposed technique.
\end{itemize}

\cs{After reading the intro, it is a bit unclear to me what does composition learning refer to in this context, and how MOREL fits composition learning.}


==> sections/backup/intro.tex <==
\section{Introduction}
\label{sec:intro}

A core problem in image retrieval is that the user has a ``concept'' in mind,
which they want to find images of, but they need to somehow convey that concept
to the algorithm. There are several ways of formulating the concept as search query,
such as a text string, a similar image, or even a sketch, or some combination of the above.
In this work,  we consider the case where queries are formulated as an input image
plus a text string that describes some desired modification to the image.
We call this task ``\fancyname'', which stands for "Image Retrieval Using Text and Image Queries".
This is closely related to attribute-based product retrieval
(see e.g.,  \cite{han2017automatic}), but differs in that the text can be multi-word,
rather than a single attribute.

We  use standard deep metric learning methods such as triplet loss
(e.g., \cite{hermans2017defense})
for computing similarity between a search
query $q_i$ and candidate images $x_j$. We represent such similarity as $s_{ij} = \fsim(q_i, x_j)$.
The main question we study is how to represent the query $q_i$ when we have two different input modalities,
namely the input image $x_i$ and the text $t_i$.

The simplest approach is to compute image features,
$\phi_x = \fimg(x)$  (e.g., using a convolutional neural network, or CNN)
and text features, $\phi_t = \ftext(t)$ (e.g., using a recurrent neural network, or RNN),
and then to concatenate them to give $\phi_{xt}^{\emptyset} = [\phi_x, \phi_t]$.
We can then post-process this representation by passing it through another (shallow) neural network,
$\phi_{xt}^w = \MLP(\phi_{xt}^{\emptyset}; w)$,  consisting of 1 or 2 nonlinear layers with parameters $w$.
This approach has been succesfully used in a lot of prior work which focuses on visual question answering,
query classification, and related tasks (see Section~\ref{sec:related} for a discussion of related work).
However, we will show that it does not work very well for retrieval, since the resulting query representation $\phi_{xt}$
is not constrained to be similar to the target image representation $\phi_j = \fimg(x_j)$.

In our approach, we use an alternative way to create representations for queries, inspired
by residual connections. In particular, we use
$\phi_{xt}^{rg} = w_g \phi_{x} \odot \sigma(\phi_{xt}^g) + w_r \phi_{xt}^r$.
where 
$\phi_{xt}^g$ is the input to an attentional or gating layer,
which is used to modify the image features $\phi_x$ in a text-dependent way,
and $\phi_{xt}^r$ is a standard concatenative representation, reshaped to match
the dimensions of the image features.
We think of $\phi_{xt}^r$ as a residual ``delta'' that is added in image feature space,
to create a representation of the compositional image-text query.
The key point is that, by design, the final representation, $\phi_{xt}^{rg}$, "lives in"
the same feature space as target images, $\phi_j=\fimg(x_j)$.\footnote{
%
It is of course possible that an end-to-end learning approach could discover this decomposition automatically; however,  manually adding in this form of inductive bias can help reduce the sample complexity,
which is an important issue since it is difficult to obtain large paired image-text datasets.
}

We show that this representation significantly helps both retrieval and classification performance on various datasets.
In particular, we improve recall @ $K$ for the Fashion-200k dataset from
 \cite{han2017automatic} from 6.3\% to 14.1\% (for $K=1$), and from 19.9\% to 42.5\% (for $K=10$).
On the MIT-States dataset, \cite{StatesAndTransformations}, we improve classification
accuracy from 14.2\%, achieved by the previous state of the art \cite{nagarajan2018attributes},
to 15.2\%.
We also introduce a new synthetic dataset, which we call "CSS" (color, shape and size),
based on the CLEVR framework \cite{johnson2017clevr},
which lets us study multi-word text queries instead of single attribute queries.
On this dataset, we once again show the improved performance coming from our novel image-text feature representation.


==> sections/backup/methods-old.tex <==
\section{Approach}

\iffalse
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{res/pipeline.png}
\end{center}
   \caption{Metric learning pipeline}
\label{fig:pipeline}
\end{figure}


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{res/composition.png}
\end{center}
   \caption{Different composition modules}
\label{fig:composition}
\end{figure}
\fi

\begin{figure*}
\begin{center}
\includegraphics[width=0.9\linewidth, ]{res/newpipeline.pdf}
\end{center}
   \caption{The system pipeline for training. We show a 2d feature space for visual simplicity.}
\label{fig:modviares}
\end{figure*}


%restate the problem setting.
Given a query image and a text description, our goal is to retrieve relevant images that are visually similar to the query image except for the modification specified in the text. The key challenge here is how to learn a meaningful visual-text compositional feature. In the rest of this section, we will first discuss our overall network architecture, then introduce a new module~\fancyname for visual-text composition, and finally discuss the training objective. 

%In addition, \fancyname is able to learn compositional embedding for classification to recognize unseen attribute combinations. We will discuss it in Section~\ref{} and empirically verify it in Section~\ref{} 


\subsection{Network Architecture}

We formulate our problem as an image-to-image retrieval problem, and employ the deep metric learning framework~\cite{wang2014learning} to tackle it. Our overall network architecture is illustrated in Fig.~\ref{fig:modviares}. As shown, a query consists of a reference image and a modification text (could be word, phrase or sentence). Both the reference image and target image are encoded by the CNN (ResNet-17) and the modification text is encoded by a standard LSTM represented by the last hidden state. During training, the network is learned, from the labeled images and text, to encode images to a compositional feature space such that metric distance in this space reflects their semantic similarity, \ie, the composition feature is closer to that of the target images but far away from others.

At test time, given a query image and a modification text, the system is used to rank a database of images, carried out by extracting composition feature of the query, and then searching for nearest neighbors in the learned feature space space. Ideally the target images should be on the top of the ranked list.

The composition module takes the input of the feature map from any layer and the LSTM latent state, and outputs the composition feature map. Of course, there exist many plausible composition mechanisms. In fact, we experimented with six representative approaches in the field of VQA and compositional learning. See Section~\ref{sec:css}. Experiments show that these approaches all lead to suboptimal results. The underlying reason may be that these approaches aim at producing a ``brand new'' feature which turns out to be difficult for image retrieval due to the considerable difference between the text and images feature.

%In experiments, we use Resnet-17 (output size = 512) as feature extractor for image and LSTM (hidden size is 512) as feature extraction for text.





%Therefore a composition module is used to embed the query. In our system, we will use the image feature CNN as part of the composition in addition to a modification via residual value process. This will be described in next section. After that, the training objective will be discussed.



\subsection{\fancyname: modification via residual link}

%\cs{Two quick questions: (1) what would be the intuition for this particular model design? (2) How does it compare with FiLM? Why would RN [33] a relevant baseline? Thanks!}
%\nam{1) what would be the intuition for this particular model design? Mostly just what I already wrote: slightly modification of the image feature instead of creating a brand new feature. Other things like weighting, gating, modification at conv level,... are basically trials and errors / implementation detail tuning. 2) How does it compare with FiLM? Very very similar to FilM and ResNet architecture (although I made it up before reading feature modulation, so can't say I was inspired by FiLM). Difference is that: [intuition] in FilM it's a way to inject text features to CNN, while my initial intention is to inject modification to the output feature (not into CNN itself). And [technical] our "modification" here is information from both image and text (instead of just text feature).
%3) Why would RN [33] a relevant baseline? maybe Lu could answer this. I do think feature modulation (FiLM) would be a relevant baseline, but Relationship network formulation doesn't look relevant to our task, so all I could say about it is that it's another way to combine image n text, and that it seems popular?}

Instead of producing a ``brand new'' feature from, another approach would be to use the image feature as the reference or context, and output it after a modification procedure, since, after all, both the features of the ``modified'' query image and the target image are expected to lie closer to each other in the learned space.

%lie in the same feature space and close to each other in some semantic perspective.
We propose a simple yet effective approach where composition is modeled as modification via residual link, as shown in the bottom of Fig.~\ref{fig:modviares}. Following the ResNet block architecture, the output feature is an element-wise sum pooling of (1) an identity connection of the input feature map, and (2) a residual connection, which is the concatenation and 2 layers feed forward network of both input. The modification is controlled by a learnable gating function, weighing the intensity of the two connections allowing the network to adapt differently to each dataset. Considering the modification may target a spatial region or the entire image, we can apply~\fancyname to the last convolution layer feature (spatial region) or the last fully-connected layer feature (entire image).

%As shown in figure \ref{fig:modviares} (bottom), the modification process can be applied to earlier feature map instead, we experiment with applying it at the last conv layer. 
%This can be useful if it needs to make use of low level image feature or spatial information.

Formally, let $\phi (x_i) \in \mathbb{R}^{W \times H \times C}$ denote the feature map for the $i$-th image obtained from any convolution or fully-connected layer, $\phi_i$ for short. For the last layer, we have $W = H = 1$. $w_i$ denotes the modification text and is encoded as $h_i \in \mathbb{R}^d$. \fancyname calculates the modified feature map from:
\begin{align}
\label{equation:morel}
\widetilde{\phi} (x_i, w_i) = w_g f_{gate} (\phi_i, h_i) + w_r  f_{res} (\phi_i, h_i),
\end{align}
where $f_{gate}, f_{res} \in \mathbb{R}^{W \times H \times C}$ are the identity and the residual connection shown in Fig.~\eqref{fig:modviares}. $w_g, w_r$ are learnable weights to balance them. The residual link is learned by two convolutional layers:
\begin{align}
f_{res} (\phi_i, h_i) = W_{r2} * relu(W_{r1} * ([\phi_i, h_i])),
\end{align}
where $*$ represents the 2D-Conv operation with the batch normalization. $[\phi_i, h] \in \mathbb{R}^{w \times h \times (c+d)}$ is the feature concatenation along the last dimension. Note that we broadcast $h_i$ along the height and width dimension so that its shape is compatible to the 3D feature map.

The identity connection is computed by:
\begin{align}
f_{gate} (\phi_i, h_i) = \sigma(W_{g2} * relu(W_{g1} *[\phi_i,  h_i])) \odot \phi_i,
\end{align}
where $\sigma$ is the sigmoid function. $\odot$ is element wise product. Similarly, $W_{g1}$ and $W_{g2}$ are 3x3 convolution filters to learn.

Eq.~\eqref{equation:morel} is designed to learn how to ``modify'' the image feature based on the text feature. The two connections have different purposes where the identity makes it easy to retain the input feature to preserve sufficient context, which is especially helpful if the modification is minor or only with respect to a certain region of the image. In comparison, the residual connection learns the delta modification to apply on the context feature. The modification value is passed through a residual link and combined with the context feature a simple sum operator.

%The gating connection makes it easy for the system to retain feature from the input image, and especially helpful if the text modification is minor or only with respect to certain region in the image. 
%\nam{I think it is better to abtract them as $nn_g$ and $nn_r$, and detail their implementation is 2 layers network. That would improve readability and correctness. Current formulation are missing activation functions and batchorm functions.}


\subsection{Deep Metric Learning}
Our training objective is to push closer the features of the ``modified'' and target image, while pull the features of non-similar images away from each other. We employ a classification loss for such objective. The input to the loss function is a batch of features, in which some pairs are labeled similar and in our case, the feature can be composition feature or image feature, and the label is that the pair of composition query and the corresponding target image is "similar").


% We sample a cluster of $k$ features from a mini-batch. For each anchor, the cluster includes a ``positive'' feature (labeled as the target images) and $k-1$ "negative" features (otherwise). Each of the positive and negative feature in this cluster will act as a nominal category whose similarity to the anchor is treated as the prediction. The overall loss equals to the average softmax cross entropy over all clusters.


% Formal definition
Formally, given a mini-batch of paired features $\{(\widetilde{\phi}^{ref}_i, \phi^+_i)\}_{i=1}^m$, where $\widetilde{\phi}^{ref}_i$  is the final modified feature computed from Eq.~\eqref{equation:morel} acting as the anchor and $\phi^+_i$ is the feature of its corresponding target image acting as positive/similar example; we also select $k-1$ image features $\phi^-_1, \cdots, \phi^-_{k-1}$ (from the other pairs in the same mini-batch) acting as negative/non-similar to the anchor. Let $\mathcal{N}$ denote $[\phi^+_i, \phi^-_1, \cdots, \phi^-_{k-1}]$, the training loss is computed using the softmax cross-entropy:

%Notice here we overload the superscript to index the reference and target images.
%represents the feature of the $i$-th reference image and $\phi^{ref}_i$
%$\widetilde{\phi}_i$, $b$ is the mini-batch size and $l$ denotes the last layer.

%\begin{align}
%L = \sum_i \sum_{j=1}^k \mathds{1}(y_j=1) \log\{\frac{\exp\{\kappa(\widetilde{\phi}^{ref}_i, \phi^+_i)\}}{\sum_{\phi_t \in \mathcal{N}^-} \exp\{\kappa(\widetilde{\phi}^{ref}_i, \widetilde{\phi}_t)\}}\},
%\end{align}

\begin{align}
\label{eq:loss_softmax}
L =  \frac{1}{M} \sum_{(i, N)} - \log\{\frac{\exp\{\kappa(\widetilde{\phi}^{ref}_i, \phi^+_i)\}}{\sum_{\phi_t \in \mathcal{N}} \exp\{\kappa(\widetilde{\phi}^{ref}_i, \phi_t)\}}\},
\end{align}
%\nam{this equation might be more accurate. inner expression is the loss over a cluster, (1/M)sigma means average over all possible cluster. Generally M might be in the order of (2m choose k+1), so it is only manageable in the extreme case of min and max value of k}

where $\kappa$ is a similarity kernel and is implemented as the dot product or the negative $l_2$ distance in our experiments. Eq.~\eqref{eq:loss_softmax} is the softmax cross entropy over a nominal class which is fixed to 1. The loss is an average over all selections of anchor, positive and negative examples, where $M$ is the number of such selection.

With smallest value $k=2$, Eq.~\eqref{eq:loss_softmax} can be easily rewritten as:
%\begin{align}
%L &= \sum_i \text{sigmoid} \{\kappa(\widetilde{\phi}^{ref}_i, \phi^+_i) - \kappa(\widetilde{\phi}^{ref}_i, \phi^-_i)\},
%\end{align}
%$[1, 0, 0, \cdots, 0] \in \{0,1\}^k$.
%each
%and ample $k-1$ features $\mathcal{N}^- =$ such that 
% add the case of multiple relevant images.
%For each pair $(\phi^l_i, \widetilde{\phi}^l_i)$, $\phi^l_i$ is called an anchor and we randomly sample $k-1 (k < b) $ images so that they are unsimilar to every anchor in the mini-batch. For every pair, we compute a similarly vector  where each:
%We found the loss fits large datasets faster \nam{no, its the other way around} and share some connection to the triplet loss~\cite{}.
\begin{align}
L =  \frac{1}{M} \sum_{(i, \phi^-)} \log\{1 + \exp\{\kappa(\widetilde{\phi}^{ref}_i, \phi^-) - \kappa(\widetilde{\phi}^{ref}_i, \phi^+_i)\}\},
\end{align}
\nam{N-becomes a single negative example, inner expression is simplified.}


As shown, this becomes the soft triplet based loss used in \cite{vo2016localizing,hermans2017defense}; in our implementation there is $M=m(m-1)$ unique selections. 
While a largest value of $k$ resembles classification based loss used in \cite{goldberger2005neighbourhood,movshovitz2017no,snell2017prototypical,gidaris2018dynamic} (in some approaches, positive or negative examples can be pre-chosen examples or replaced with learnable weights); in this case $M=m$. In our experience, the later case becomes more discriminative and fits faster, but can be more vulnerable to overfitting.

At test time, composition and image are embeded in the same feature space allowing retrieval by nearest neighbor search. In our image retrieval experiment, the task is to search for similar images in this space given the composition feature as query.



==> sections/backup/methods.tex <==
\section{Method}
\label{sec:method}


\iffalse
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{res/pipeline.png}
\end{center}
   \caption{Metric learning pipeline}
\label{fig:pipeline}
\end{figure}


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{res/composition.png}
\end{center}
   \caption{Different composition modules}
\label{fig:composition}
\end{figure}
\fi

\begin{figure*}
\begin{center}
\includegraphics[width=0.9\linewidth, ]{res/newpipeline.pdf}
\end{center}
   \caption{The system pipeline for training. We show a 2d feature space for visual simplicity.}
\label{fig:modviares}
\end{figure*}


As explained in the introduction, our goal is to learn an embedding space for the text+image query and for target images,
such that matching (query, image) pairs are close.  Our overall network architecture is illustrated in Fig.~\ref{fig:modviares},
and is explained in more detail below.

%\subsection{Computing image and text features}
\subsection{Proposed method for combining image and text}

First we encode the query image $x$ using a ResNet-17 CNN to get a 2d spatial feature vector $\phi_x \in \mathbb{R}^{W \times H \times C}$,
where $W$ is the width, $H$ is the height, and $C=512$ is the number of feature channels.
%For Fashion200k and MIT-States, we use the final layer, so $W=H=1$, 
%whereas for CSS, we use the penultimate later, so $W=H=?$. \km{Fill in details.}
Next we encode the query text $t$ using a standard LSTM. We define $\phi_t$ to be the hidden state at the final time step.
(We could also use a bidirectional LSTM, but since the strings are short, this does not make much difference.)

We now combine image and text features using
\begin{align}
\label{equation:morel}
\phi_{xt}^{rg}
= w_g \fgate (\phi_x, \phi_t) + w_r  \fres (\phi_x, \phi_t),
\end{align}
where $\fgate, \fres \in \mathbb{R}^{W \times H \times C}$ are the gating and the residual connection shown in Fig.~\eqref{fig:modviares}. $w_g, w_r$ are learnable weights to balance them. 
The gating connection is computed by:
\begin{align}
\fgate(\phi_x,\phi_t) = \sigma(W_{g2} * \relu(W_{g1} *[\phi_x,  \phi_t]) \odot \phi_x
\end{align}
where $\sigma$ is the sigmoid function, $\odot$ is element wise product,
 $*$ represents  2D convolution with  batch normalization,
and $W_{g1}$ and $W_{g2}$ are 3x3 convolution filters.
Note that we broadcast $\phi_t$ along the height and width dimension so that its shape is compatible to the image feature map $\phi_x$.
The residual connection is computed by:
\begin{align}
\fres(\phi_x, \phi_t) = W_{r2} * \relu(W_{r1} * ([\phi_x, \phi_t])),
\end{align}
Eq.~\eqref{equation:morel} combines these two feature vectors using addition.
The intuition is that we just want to ``modify'' the image feature based on the text feature,
rather than create an entirely different feature space.
If we use the fully connected (non-spatial) layer of the image feature extractor,
we are modifying global properties of the representation,
whereas if we use a spatial image feature map, we can modify pieces of the image in a more local way.
\lu{todo: discuss the special case on the fc layer.}
\nam{a}
%We will see below that different datasets require different forms of featyures.

\subsection{Existing methods for combining image and text}


We implement the following composition mechanisms as our baselines\footnote{
%
It is of course possible that an end-to-end learning approach could discover this decomposition automatically; however, manually adding in this form of inductive bias can help reduce the sample complexity,
which is an important issue since it is difficult to obtain large paired image-text datasets.
}
:
\begin{itemize}
   \item \textbf{Image Only}: we set $\phi_{xt}=\phi_x$.
   \item \textbf{Text Only}: we set $\phi_{xt}=\phi_t$.
   
   \item \textbf{Concatenate} computes $\phi_{xt} = W_{2} * \relu(W_{1} *[\phi_x,  \phi_t]$.
   This has  been used in a variety of applications such as VQA~\cite{vqa}, dialog-based image search~\cite{guo2018dialog},  attribute manipulation image search~\cite{zhao2017memory}, etc.
   \km{Is this correct? Or do you just use $\phi_{xt}= [\phi_x, \phi_t]$?} \nam{correct, though I do have additional dropout 0.1 and batchnorm in there.}
   
   \item \textbf{Show and Tell}~\cite{vinyals2015show}. In this approach, we train an image-conditioned LSTM to generate the text $t$ given $x$. We use the final state of this LSTM as our representation $\phi_{xt}$.
   
   \item \textbf Attribute as Operator \cite{nagarajan2018attributes} embeds each text attribute as a transformation matrix, $T_t$,
   and applies $T_t$ to $\phi_x$ to create $\phi_{xt}$.

   \item \textbf{Parameter hashing}~\cite{noh2016image} is a technique proposed for VQA task. In our implementation, it modifies the query image representation by injecting text feature into the image CNN as parameters of one fully connected layer.
   \km{Explain this in more detail.}
  
   \item \textbf{FiLM}~\cite{perez2017film} is a technique proposed for VQA task. The text feature is injected into the image CNN additively for the residual connections and multiplicatively for the gating connections.
   This is similar to our approach, except they modify every layer on the image feature stack, whereas we only modify the final output.
   \km{Is it true that the only difference from FILM is that you modify 1 layer and they modify all layers? This is a rather trivial difference...}
   \nam{Yes, the difference is very small. But somewhat significant at the same time because the design goals and what they actually do is different. FiLM tries to inject text into a CNN, changing the internal structure and also final feature space. Our goal is to not change the (pretrained) CNN, hence keeping the meaningful image feature space the same and perform modification within. On the technical side, both use resnet block and gating, which are existing techniques, that is how I made it up before knowing FiLM. imo the biggest contribution of FiLM paper is not this modification (or modulation as they call it), but the fact that it is applied to all layers.}
  
   \item \textbf{Relationship}~\cite{santoro2017simple} is another technique proposed for VQA task, where the text feature is injected by concatenation. This architecture has the ability to relate pairs of regions in the image hence can learn the relationship information.
 \km{explain this in more detail}
\end{itemize}

For a fair comparison, all baselines including ours are trained using the same pipeline, with the only difference being in the composition module.


%The gating connection makes it easy for the system to retain feature from the input image, and especially helpful if the text modification is minor or only with respect to certain region in the image. 
%\nam{I think it is better to abtract them as $nn_g$ and $nn_r$, and detail their implementation is 2 layers network. That would improve readability and correctness. Current formulation are missing activation functions and batchorm functions.}


\subsection{Deep Metric Learning}
\label{sec:DML}


%\newcommand{\query}{\widetilde{\phi}^{ref}_i}
\newcommand{\query}{\psi_i}

Our training objective is to push closer the features of the ``modified'' and target image, while pulling apart the features of non-similar images. We employ a classification loss for this task. More precisely,
the input to the loss function is a batch of features, in which some pairs are labeled similar.
More precisely, suppose we have a minibatch of $B$ feature vectors,
where $\phi_i=\fimg(x_i)$ is the representation for the $i$'th image,
and $\query=\fquery(x_i, t_i)$ is the modified representation for that image.
We use $\phi_i^+$ to denote the feature vector for the image that matches query $i$.
For each query $i$,
we create a set of $K-1$ negative examples, $\mathcal{N}_i = [\phi_{1}^-,\ldots, \phi_{K-1}^-]$, by sampling from the minibatch
excluding $\phi_i$.
We repeat this $M$ times to get sets $\mathcal{N}_i^m$.
We then define the following softmax cross-entropy loss:

\begin{align}
\label{eq:loss_softmax}
L =  \frac{1}{MB} \sum_{i=1}^B \sum_{m=1}^M - \log\{\frac{\exp\{\query, \phi^+_i)\}}
{\sum_{\phi_j^- \in \mathcal{N}_i^m} \exp\{\kappa(\query, \phi_j^-)\}}\},
\end{align}
%\nam{this equation might be more accurate. inner expression is the loss over a cluster, (1/M)sigma means average over all possible cluster. Generally M might be in the order of (2m choose k+1), so it is only manageable in the extreme case of min and max value of k}
where $\kappa$ is a similarity kernel and is implemented as the dot product or the negative $l_2$ distance in our experiments. %Eq.~\eqref{eq:loss_softmax} is the softmax cross entropy over a nominal class which is fixed to 1. The loss is an average over all selections of anchor, positive and negative examples, where $M$ is the number of such selection.
When we use the smallest value of $K=2$, Eq.~\eqref{eq:loss_softmax} can be easily rewritten as:
%\begin{align}
%L &= \sum_i \text{sigmoid} \{\kappa(\widetilde{\phi}^{ref}_i, \phi^+_i) - \kappa(\widetilde{\phi}^{ref}_i, \phi^-_i)\},
%\end{align}
%$[1, 0, 0, \cdots, 0] \in \{0,1\}^k$.
%each
%and ample $k-1$ features $\mathcal{N}^- =$ such that 
% add the case of multiple relevant images.
%For each pair $(\phi^l_i, \widetilde{\phi}^l_i)$, $\phi^l_i$ is called an anchor and we randomly sample $k-1 (k < b) $ images so that they are unsimilar to every anchor in the mini-batch. For every pair, we compute a similarly vector  where each:
%We found the loss fits large datasets faster \nam{no, its the other way around} and share some connection to the triplet loss~\cite{}.
\begin{align}
L =  \frac{1}{MB} \sum_{i=1}^B \sum_{m=1}^M \log\{1 + \exp\{\kappa(\query, \phi_{i,m}^{-}) - \kappa(\query, \phi^+_i)\}\},
\end{align}
since each set $\mathcal{N}_i^m$ contains a single negative example.
This is equivalent to the the soft triplet based loss used in \cite{vo2016localizing,hermans2017defense}.
We use $M=m(m-1)$ so we pair each example $i$ with all possible negatives.
If we use larger $K$, each example is contrasted with a set of other negatives;
this loss resembles the classification based loss used in \cite{goldberger2005neighbourhood,movshovitz2017no,snell2017prototypical,gidaris2018dynamic}.
In this case, we use $M=m$ negative sets.
In our experience, this  case is more discriminative and fits faster, but can be more vulnerable to overfitting.
\km{Did I get the equations right?} \nam{for a valid softmax, N includes both positive and negatives. Another note is that we want to look at all possible N, and then M can get exponentially big. Thats why in my implementation, it is just extreme value of K so that M is managable.}





==> sections/backup/related-old.tex <==
\section{Related work}
\label{sec:related}

% \lu{summary of our previous discussions: 1) difference to attribute composition: 1 shot and cross-model. 2) difference to fashion search: attribute versus phrase (more complicated) ; open versus closed vocabulary; 3) difference to conditional GAN: modify at the feature space other than at the pixel space.}
\textbf{Compositional Learning}:
Representing new concept via a novel combination of attribute values has been studied in previous works on zero-shot learning such as \cite{lampert2009learning, romera2015embarrassingly,zhang2015zero}. Differently we study composition of image and text; in this context the text is concepts seen during training and the image represent new concept at test time that needs to be 1 shot learnt.
In \cite{misra2017red}, Misra et al investigate learning a composition classifier by combining existing object classifier and state classifier. It is shown that novel composition classifiers can be generated at test time. Nagarajan at al \cite{nagarajan2018attributes} proposed an embedding approach where the composition is formalized as dot product operation between the object embedding and the state transformation matrix. 
% Inspired by these works, we adapt their compositional techniques as baselines for our task of image text composition image search.
\lu{add the difference to our work. 1) difference to attribute composition: 1 shot and cross-model} \nam{done}


\textbf{Vision and language}:
Our task can be considered in the topic of vision and language joint understanding: making prediction taking image and text as inputs. A notable example in this area is Visual Question Understanding (VQA) \cite{vqa, johnson2017clevr}; many techniques have been proposed to leverage and combine the 2 inputs effectively \cite{noh2016image, perez2017film, santoro2017simple}. In \cite{noh2016image}, text feature is incorporated by mapping into parameters of a fully connected layer within the image CNN. Feature modulation FiLM \cite{perez2017film} injects text feature into image CNN at all layers via addictive connections (residual \cite{he2016deep}) and multiplicative connections (gating \cite{miech2017learnable}). Our method uses the same operations but only at the output level layer since our goal is to modify the query image representation, and contain that process within the same already meaningful image feature space. In contrast, FiLM, together with other baseline methods that we study, learns a new representation when combining image and text.
\lu{add the difference to our work.  attribute versus phrase (more complicated) ; open versus closed vocabulary;}
\nam{not applicable}
\lu{add difference to FilM suggested by Chen}.
\nam{done}


\textbf{Conditional Generative Adversarial Nets}:
Image generation by GAN \cite{goodfellow2014generative} has been a very popular topic. In particular conditional GAN \cite{mirza2014conditional} can be used to, from input image, generate new image with a different style, attribute value or in a different domain \cite{lample2017fader, pix2pix2017,zhu2017unpaired,choi2018stargan}. 
Note that our task is image retrieval, so we're not synthesizing the image~\lu{why}~\nam{for efficiency and accuracy, image retrieval have been done by comparing feature, not image pixels, so likely the reviewers are not gonna ask}, but a feature that will help to retrieve the desired image correctly. 


\textbf{Image retrieval and product search}:
Image retrieval is an important vision problem and significant progress has been made thanks to deep learning \cite{chopra2005learning, wang2014learning}; it has numerous applications such as product search \cite{liu2016deepfashion}, face recognition \cite{schroff2015facenet} or image geolocalization \cite{hays2008im2gps}. Cross modality image retrieval allows using other types of query, examples include text to image retrieval \cite{wang2016learning}, sketch to image retrieval \cite{sangkloy2016sketchy} or cross view image retrieval \cite{lin2015learning}. We consider our set up an image to image retrieval task, but the image query is augmented with an additional modification text input.


A lot of research has been done to improve product retrieval performance by incorporate user's feedback to the search query in the form of relevance \cite{rui1998relevance}, relative \cite{kovashka2012whittlesearch} or absolute attribute \cite{zhao2017memory, han2017automatic, ak2018learning}. Tackling the problem of image based fashion search, Zhao et al \cite{zhao2017memory} proposed a memory-augmented deep learning system that can perform attribute manipulation. In \cite{han2017automatic}, spatially-aware attributes are automatically learned from product description labels and used to facilitate attribute-feedback product retrieval application. We're approaching the same image search task, but incorporating text into the query instead, which can be potentially more flexible than using a predefined set of attribute values.

Parallel to our work is Dialog-based Interactive Image Retrieval \cite{guo2018dialog}, where Guo et al explore using natural language as input feedback to improve image retrieval result. Their proposed reinforcement learning system demonstrates promising result on simulated user and real world user study. Though the task is similar, their study focuses on modeling the interaction between user and the agent; meanwhile we study and benchmark different image text composition mechanisms.


==> sections/backup/results-old.tex <==
\section{Experiments}

We evaluate the proposed model on three datasets: Fashion200k~\cite{han2017automatic} and MIT-States~\cite{StatesAndTransformations}, and a new dataset called CSS. The retrieval task on these datasets requires effective composition between texts and images, and are of great importance with many applications in image search and product search. While Fashion200k~\cite{han2017automatic} and MIT-States~\cite{StatesAndTransformations} are actually for attribute feedback task, CSS is designed for text feedback and therefore the main one we use to study and analyze. We demonstrate that \fancyname performs favorably against the state-of-the-art models on these datasets. The source code, CSS dataset, and trained models will be made available to the public.


%They are technically attribute feedback/modification image search; we will treat attribute as text when applying our method.

%\lu{Add the filter size and stride info in experimental sections}.

\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{res/cssqual2.png}
\end{center}
   \caption{Some retrieval examples on CSS Dataset.}
\label{fig:cssqual}
\end{figure*}


\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{res/cssreconstruction3.png}
\end{center}
   \caption{Reconstruction images from the learned composition features.\lu{put the name on top of each method and align them vertically}}
   %\lu{find a better example for the second and third row. maybe few objects? This figure is very  important.}} \nam{done. Though I think we should not cherry pick, most reconstruction is not 100 accurate, especially I still think this visualization is not very meaningful anyway}
\label{fig:cssreconstruction}
\end{figure*}


\subsection{CSS dataset}\label{sec:css}

\noindent\textbf{Dataset}: Since existing benchmarks for image retrieval may not contain complex text modifications, we establish a dataset using the CLEVR toolkit~\cite{johnson2017clevr} for generating synthesized images in a 3-by-3 grid scene in which objects with different \emph{C}olor, \emph{S}hape and \emph{S}ize (CSS) occupy. Each image comes in a simple 2D blobs version and a 3D rendered version. Examples are shown in Fig.~\ref{fig:cssqual}. We generate three types of modification texts from templates: adding, removing or changing object attributes. In total, there are 16k queries for training and 16k queries for test. Each query is of a reference image (2D or 3D) and a modification, and the target image. More details are available in the supplementary material. Note CSS dataset is one-of-the-first benchmarks for studying compositional learning for image retrieval. It allows us to control the task complexity and diagnose of the results by configuring settings of image types (2D or 3D) and modification types (add, remove or modify). 


\noindent\textbf{Metrics and Baseline}: Recall at rank k (R@k) is employed as the metric for retrieval, computed as the percentage of test queries where (at least 1) target or correct labeled image is within the top k retrieved images. Each experiment is repeated 5 times to obtain a stable retrieval performance, and both mean and standard deviation are reported.



We implement the following composition mechanisms as our baseline:
\begin{itemize}
   \vspace{-2mm}
   \item \textbf{Image Only} or \textbf{Text Only}: just the image feature or the text feature is used as the composition feature.
   \vspace{-2mm}
   \item \textbf{Concatenate} is a very simple way that concatenates image features and text features, followed by a 2 layers feed forward network. It has been used in a variety of applications such as VQA~\cite{vqa}, dialog-based image search~\cite{guo2018dialog},  attribute manipulation image search~\cite{zhao2017memory}, etc.
   \vspace{-2mm}
   \item \textbf{Show and Tell}~\cite{vinyals2015show} is well-known for image captioning: the query image feature is first fed into a LSTM, and then followed by each of the word in the text, at each step the network predicts the next word. We adapt it for this task by using the LSTM's last output as the image text composition feature.
   \vspace{-2mm}
   \item \textbf{Attribute as Operator}~\cite{nagarajan2018attributes} embeds each attribute as a transformation matrix and modification is carried out by applying that transformation to the image feature vector.
   \vspace{-2mm}
   \item \textbf{Parameter hashing}~\cite{noh2016image} is a technique proposed for VQA task. In our implementation, it modifies the query image representation by injecting text feature into the image CNN as parameters of one fully connected layer.
   \vspace{-2mm}
   \item \textbf{FiLM}~\cite{perez2017film} is a technique proposed for VQA task. The text feature is injected into the image CNN through modulation operation. 
   %(addictively by residual connections and multiplicative by gating connections)
   \vspace{-2mm}
   \item \textbf{Relationship}~\cite{santoro2017simple} is another technique proposed for VQA task, where the text feature is injected by concatenation. This architecture has the ability to relate pairs of regions in the image hence can learn the relationship information.
   \vspace{-2mm}
\end{itemize}

For a fair comparison, all baselines including ours are trained using the same pipeline with only difference in the composition module.

%between different composition mechanisms. 

\noindent\textbf{Implementation Details}: In PyTorch, we use ResNet-17 (output feature size = 512) as feature extractor for image and LSTM (hidden size is 512) as feature extraction for text. The modification process is applied to either the final feature output of the image CNN (Fashion200k and MIT-States) or the penultimate feature map (CSS Dataset). The DML loss function with $k=2$. Training is run for 150k iterations with learning rate 0.01. 
%\lu{add more details. Look at papers in ICLR and see what do they report, e.g. filter size end etc.} \nam{done}


\noindent\textbf{Main Results}: Table~\ref{tab:css} summarizes R@1 retrieval performance on the CSS dataset. We examine two retrieval settings using the 3D reference image (2nd column) and the 2D image (3rd column). As shown, our method performs well against the state-of-the-art methods in both settings, improving the best baseline by a relative 6-12\%. The results show that \fancyname is effective for compositional visual-text learning for image retrieval. Fig.~\ref{fig:cssqual} plots some queries and retrieved image by our method. As we see, the  2D-to-3D setting is quite challenging which uses a 2D image and a text to search the database of 3D images. Nevertheless, our method is able to find reasonable results. Notice that we use separate encoders to extract features for 2D and 3D images in this setting.

%Some qualitative example are shown in figure \ref{fig:cssqual}. The top rows are successful retrieval cases for each of the 3 types of modifications (add, remove and change), the last row shows a failure example.
%R@1 retrieval performance is shown in table \ref{tab:css}. Our approach of modifying image representation via residual value outperforms the baselines.

%Cross domain retrieval result (2D to 3D): we also experiment with a setting where the image used in the query is the 2D version and the goal is to retrieve from the database of 3D images. 

%This cross domain retrieval setting is more challenging, resembling cross-view or sketch to natural image search. The training pipeline is still the same, only now different encoders are used to extract features from 2D and 3D images. The result is shown in table \ref{tab:css}, right column. Our method achieves better performance in this setting too.

To visualize the learned composition features, we first train a transposed convolutional network to reconstruct the images from their features, and then apply it to the composition feature. Fig.~\ref{fig:cssreconstruction} shows the reconstructed images from the composition features of three methods, in which the images are blurry as we use the regression loss to train the network. Note a nicer reconstruction may not mean better retrieval performance, as the composition feature is learned to capture the discriminative information to find the target image.

As we see, our method captures essential attributes about the query including changes to an object's color, position and shape. Comparatively, our reconstruction results are more sensible to humans, suggesting that the learned composition is semantically meaningful. We attribute this to our proposed architecture which allows composition features to be more effectively learned by modification through the residual connection.

%In comparison, baseline composition feature with
%However it is good enough to verify that the feature correctly captures essential information of the scene (object's position and their color, size, shape attribute).
%We will compare with the concat fusion baseline. As shown in figure \ref{fig:cssreconstruction}, even though the reconstructions from both our and baseline composition feature don't look the same as the target, the baseline are less accurate (for example color of existing objects are often changed). We argue this is due to the identity connection, our method can retain a lot of information from the query image feature and is able to produce a similar type of feature, hence closer reconstruction. We note that this is purely visualization; a nicer reconstruction does not mean better retrieval performance; the composition feature only need to capture enough information to allow it to be discriminate.




\begin{table}
\centering
\begin{tabular}{|l|c|c|}
\hline
Method & 3D-to-3D & 2D-to-3D \\
\hline\hline
Image only & 6.3 & 6.3 \\
Text only & 0.1 & 0.1 \\
\hline
Concatenate & 60.6$^{\pm0.8}$ & 27.3 \\
Show and Tell & 33.0$^{\pm3.2}$ & 6.0 \\
Parameter hashing & 60.5$^{\pm1.9}$ & 31.4 \\
Relationship \cite{santoro2017simple} & 62.1$^{\pm1.2}$ & 30.6 \\
FiLM \cite{perez2017film} & 65.6$^{\pm0.5}$ & 43.7 \\
Ours &  \textbf{73.7}$^{\pm1.0}$ & \textbf{46.6} \\
\hline
\end{tabular}
\caption{Retrieval performance (R@1) on CSS Dataset.\lu{no std on 2D-to-3D?} \nam{will need to do more runs to get std, I'll start once the current exp is done.}}
\label{tab:css}
\end{table}



\subsection{Fashion200k}

Fashion200k ia a challenging dataset~\cite{han2017automatic} consisting of $\sim$200k images of fashion products. Each image comes with a compact attribute description (such as black biker jacket or wide leg culottes trouser).
Following~\cite{han2017automatic}, queries are created as following: pairs of products that have one word difference in their descriptions are selected as the reference images and target images; 
and the modification text is that one different word and is used as an input together with the reference image. We benchmark on this task by treating the product image and the attribute as a compositional query. In total, we have xxx queries for training and 3,167 for validation. To compare with~\cite{han2017automatic}, we randomly sample 10 validation sets and report the mean \footnote{We contacted the authors of~\cite{han2017automatic} for the original 3,167 test queries, but got only the product descriptions. We attempted to recover the set from the description. However, on average, there are about 3 product images for each unique product description.}. The queries allow users to conduct attribute-feedback product retrieval \cite{kovashka2012whittlesearch, zhao2017memory, han2017automatic, ak2018learning} and are of great importance for product search application.

%\lu{can you find more numbers on this dataset from https://scholar.google.com/scholar?um=1&ie=UTF-8&lr&cites=2145472419470460203}
%\nam{didn't find anything on that site, and Im pretty sure there's no numbers reported for that dataset because it is new and even the author does not have the testset}

%The training data is generated by a similar procedure on the train split of Fashion200k. Note that the set of test queries might not be exactly the same. We contacted authors of \cite{han2017automatic} to get the original 3,167 queries; unfortunately only the product descriptions  are available. Based on that, we attempted to recreate this test set; however on average, there is 3 product images for each unique product description. To make the result as comparable as possible, we sample 10 test sets like that, test on all of them and report the mean.

%To generate training data for our system, we perform similar procedure but on the train split of the dataset.


Table~\ref{tab:f200k} shows the results, where the recall of the first row is from~\cite{han2017automatic} and the others are from our framework. We have two observations. First, our method significantly improve the \cite{han2017automatic} demonstrating the efficacy of our learning framework. In our speculation, it is mainly because \cite{han2017automatic} trained with a image-text embedding objective which might be less optimal for the retrieval task. Second, our method outperforms all baseline with statistical significance, which is consistent with the result on the CSS dataset. This demonstrates the advantage of modification via residual link over other composition mechanisms that aims to produce a new feature from input. Some qualitative retrieval examples are shown in Fig.~\ref{fig:f200kqual}. 
%R@k retrieval performance are reported in table \ref{tab:f200k}.

%It achieves the best-published retrieval on Fashion200k.

\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{res/f200kqual.png}
\caption{Retrieval examples on Fashion200k dataset. (nam: will change to original images later)}
\label{fig:f200kqual}
\end{figure*}


%Compared to the baselines from \cite{han2017automatic}, our method and baseline is significantly better. In our speculation, it is mainly because \cite{han2017automatic} train with a image text embedding objective which might not be optimial for this retrieval task. There is also difference in backbone architecture: methods in \cite{han2017automatic} uses InceptionV3 while we use the ResNet-17.

%Compared to the concat fusion NN baseline, our is also slightly better. Consistent with the result on CSS dataset, this shows that modification via residual value have the advantage compared to composition method that tries to produce a new feature from input.


\begin{table}
\centering
\begin{tabular}{|l|ccc|}
\hline
Method & R@1 & R@10 & R@50 \\
\hline\hline
%Best baseline from \cite{han2017automatic} & 6.0 & 17.0 & 37.0 \\
Han \etal~\cite{han2017automatic} & 6.3 & 19.9 & 38.3 \\
\hline
%\hline
%Image only & 3.5 & 22.7 & 43.7 \\
%Text only & 1.0 & 12.3 & 21.8 \\
Concatenation & 11.9$^{\pm1.0}$ & 39.7$^{\pm1.0}$ & 62.6$^{\pm0.7}$ \\
Show and Tell~\cite{} & 12.3$^{\pm1.1}$ & 40.2$^{\pm1.7}$ & 61.8$^{\pm0.9}$ \\
Param Hashing & 12.2$^{\pm1.1}$ & 40.0$^{\pm1.1}$ & 61.7$^{\pm0.8}$ \\
Relationship~\cite{santoro2017simple} & 13.0$^{\pm0.0}$ & 40.5$^{\pm0.0}$ & 62.4$^{\pm0.0}$ \\
FiLM~\cite{perez2017film}  & 12.9$^{\pm0.7}$ & 39.5$^{\pm2.1}$ & 61.9$^{\pm1.9}$ \\
Ours & \textbf{14.1}$^{\pm0.6}$ & \textbf{42.5}$^{\pm0.7}$ & \textbf{63.8}$^{\pm0.8}$ \\
\hline
\end{tabular}
\caption{Retrieval performance on Fashion200k.}
\label{tab:f200k}
\end{table}




\subsection{MIT-States}

MIT-States~\cite{StatesAndTransformations} is a primary benchmark for compositional learning~\cite{misra2017red,nagarajan2018attributes}. It has $\sim$60k images, each comes with an object/noun label and a state/adjective label (such as ``red tomato'' or ``new camera''). There is 245 nouns and 115 adjectives, on average each noun is only modified by $\sim$9 adjectives it affords. Previous work benchmarks on a classification setting, where a composition model is learned to recognize unseen pairs of state + noun in training. For example, training on ``red wine'' and ``old tomato'' to predict ``red tomato'' where there exist zero ``red tomato'' images in training.


% This task requires the network to learn about state/adjective (modification text) during training and to generalize to novel types of object/noun at test time. \nam{no, for classification task, all nouns and adjectives are seen in training, novel composition in test time}

For an apple-to-apple comparison to previous work, we benchmark on this compositional recognition task. It differs from our previous retrieval tasks in that (i) composition is between an object label and a state label instead of an images and a text; (ii) since it is a classification task, given an image and a modification text, the output is a label instead of a ranked list of images. To do so, we train our model the other way around to search for the most relevant class label given the image feature as query. Training procedure is also adjusted for fair comparison with~\cite{misra2017red, nagarajan2018attributes}: the same ``novel pairs'' split is used and the same ResNet-17 is employed but not fine-tuned during training.
\lu{what features do you use to represent the class label?} \nam{same as Attribute as Operator and other Label embedding baselines, I just change the composition mechanism.}

%it is a classification task: given the image output the composition label (instead of given the composition, retrieve the image).
%We also do a classification experiment where it's other way around: the task is to search for the most relevant composition given the image feature as query.

The classification accuracy is reported in Table~\ref{tab:mitstatesclassification}, where the baseline numbers are cited from the relevant papers~\cite{misra2017red,nagarajan2018attributes}. As we see, even though our method is not designed for compositional learning for classification, our method performs favorably against the state-of-the-art models, achieving the best-published accuracy on this benchmark. The results substantiate our method's efficacy for compositional learning on a different classification setting. We also create an image retrieval setting using this dataset and benchmark different baselines, result is reported in supplementary materials.

%Although not the problem we study, our method still performs decently on this composition task.


\begin{table}
\centering
\begin{tabular}{|l|c|}
\hline
Method & Accuracy \\
\hline\hline
%Chance & 0.1 \\
%Analogous Attr~\cite{chen2014inferring} & 1.4 \\
Misra \etal 2017~\cite{misra2017red} & 13.1 \\
Nagarajan \etal 2018~\cite{nagarajan2018attributes}  & 14.2 \\
Label Embedded+ & 14.8 \\
VisProd (NN) & 13.9 \\
Ours & \textbf{15.2} \\
\hline
\end{tabular}
\caption{Classification accuracy of unseen (attribute, object) pairs on MIT-States. Baseline numbers are cited from~\cite{misra2017red,nagarajan2018attributes}.} 
%\lu{not important: any chance to find a better model to report?} \nam{I think one of the model I had is slightly better, but it is a baseline model, concatenation or something}
\label{tab:mitstatesclassification}
\end{table}




\subsection{Ablation Studies}


\begin{table}[ht]
\centering
\small
\begin{tabular}{|l|ccc|}
\hline
Method     & CSS & Fashion200K & MIT-States \\
\hline\hline
\fancyname & 73.7  &   14.1    &       12.1     \\
 - w/o residue    & 06.3 &   03.5      & 03.3  \\
 - w/o identity    & 60.6 &  11.9     &  11.8 \\
 \hline
 - mod. last fc    & 71.2  &  14.1      &  12.1 \\
 - mod. last conv    &  73.7  &  12.4    &  10.3 \\
 \hline
 DML loss, k=min    & 73.7  &    10.0     &  12.1 \\
 DML loss, k=max    & 72.0 &    14.1    &  12.0 \\
\hline
\end{tabular}
\caption{R@1 of Ablation Studies.}
\end{table}



\lu{let's organize the ablation studies by 3 questions}



We perform ablation studies and report in table 4. 

\noindent\textbf{Efficacy of modification by residue connection}: our composition module is basically a ResNet block, if either the identity or the residual connection is removed, it becomes an identity operation (Image only) or the concatenate baseline, both have lower performance. 

\noindent\textbf{Efficacy of spatial-aware modification}: as our motivation is to modify the image feature but still keep it in the already meaningful feature space, our modification process is applied to the last fc layer feature, which yields competitive performance compared to baselines on all 3 datasets. Applying MOREL to the last conv feature map instead actually degrades the performance, except on CSS. In our speculation, it is because the modification here is more low level and regional. 

\noindent\textbf{The impact of $k$ on loss function}: we use k=2 (soft triplet loss) in most experiments. Fashion200k is much bigger dataset and also more challenging, we found that the system underfitted. In this case by using bigger k (same as batch size in our experiment), the system fits well and produces better result. On the other 2 datasets, it  overfits the training data, and test time performance is comparable but becomes less stable. Note that the validation here is to improve our metric learning pipeline and doesn't reflect the difference between image text composition methods.


%\subsection{Novel composition recognition result on MIT-States}
%In order to have an apple to apple comparison to previous works, we benchmark on the novel composition recognition task done in \cite{misra2017red, nagarajan2018attributes}. It differs from the previous benchmark because: (1) composition is between object label and state label (instead of object image and state label), and (2) it is a classification task: given the image output the composition label (instead of given the composition, retrieve the image).
%We can still approach this task under retrieval (i.e. classification based on nearest neighbor, similar to \cite{nagarajan2018attributes}). To do so, we adapt our composition module for object label and state label composition, and reverse the retrieval direction. Training procedure is also adjusted for fair comparison with \cite{misra2017red, nagarajan2018attributes}: the same "novel pairs" split is used, the same Resnet-17 is employed but not finetuned during training.

